Bridging the Narrative Divide: Cross-Platform Discourse Networks in Fragmented Ecosystems

Political discourse has grown increasingly fragmented across different social platforms, making it challenging to trace how narratives spread and evolve within such a fragmented information ecosystem. Reconstructing social graphs and information diffusion networks is challenging, and available strategies typically depend on platform-specific features and behavioral signals which are often incompatible across systems and increasingly restricted. To address these challenges, we present a platform-agnostic framework that allows to accurately and efficiently reconstruct the underlying social graph of users' cross-platform interactions, based on discovering latent narratives and users' participation therein. Our method achieves state-of-the-art performance in key network-based tasks: information operation detection, ideological stance prediction, and cross-platform engagement prediction$\unicode{x2013}$$\unicode{x2013}$while requiring significantly less data than existing alternatives and capturing a broader set of users. When applied to cross-platform information dynamics between Truth Social and X (formerly Twitter), our framework reveals a small, mixed-platform group of $\textit{bridge users}$, comprising just 0.33% of users and 2.14% of posts, who introduce nearly 70% of $\textit{migrating narratives}$ to the receiving platform. These findings offer a structural lens for anticipating how narratives traverse fragmented information ecosystems, with implications for cross-platform governance, content moderation, and policy interventions.

==> problem.tex <==
\section{Problem Description}

Given a set of users $U = \{u_1, u_2, ..., u_n\}$ and their associated content $C = \{c_1, c_2, ..., c_m\}$, our objective is to construct a network that captures alignment in content engagement patterns between users in a platform-agnostic manner. We formalize this as the construction of a weighted, undirected graph $G = (V, E, w)$, where:

\begin{itemize}
    \item $V \subseteq U$ is the set of nodes representing users.
    \item $E \subseteq \{(u, v) \mid u, v \in V, u \neq v\}$ is the set of edges indicating inferred relationships between users.
    \item $w: E \rightarrow [0,1]$ assigns a weight to each edge, representing the strength of behavioral alignment between users.
\end{itemize}

Unlike traditional approaches that rely on explicit network structures (e.g., follows, reposts) or direct content similarity, we infer user relationships through shared content engagement patterns. This requires network construction to remain independent of platform-specific features for generalization across different ecosystems. Additionally, edge weights $w(e)$ must maintain temporal coherence, capturing sustained behavioral alignment rather than momentary interactions. Finally, between any two users,  $w(e)$ should reflect genuine behavioral fidelity, distinguishing meaningful engagement from superficial similarity or fleeting trends.


We thus construct a cross-platform, behavior-driven user network that is resilient to platform fragmentation and effective for predictive and analytical applications. To evaluate our network construction method, we assess its performance on traditional downstream tasks such as user stance prediction and coordination detection. We further test its ability to predict future user behavior across platforms, providing insight into information diffusion and social interactions over time. 


\begin{figure*}[t] % 't' positions the figure at the top of the page
    \centering % Centers the figure horizontally
    \begin{overpic}[width=0.95\textwidth]{plots/cane-system.pdf} % Adjust the width as needed
    \end{overpic}

    \vspace{-1mm} % Reduces the vertical space by 1 millimeter
    \caption{This illustration outlines the key components of our method, which enables cross-platform user network inference. Content Aggregation processes and embeds user-generated content. Content Clustering groups semantically similar content, forming the basis for User Network Construction. The resulting networks are then broadly applicable to a wide range of social network analysis tasks, including narrative tracking, bot detection, and influence campaign analysis (we show Community Detection, Stance Prediction, and Content Distribution Analysis as examples of downstream tasks).} 
    \vspace{-3mm} % Reduces the vertical space by 3 millimeters
    \label{fig:user-network-generation}
\end{figure*}




==> time-complexity.tex <==


